The HSIC Bottleneck: Deep Learning without Back-Propagation

We introduce the HSIC (Hilbert-Schmidt independence criterion) bottleneck for training deep neural networks. The HSIC bottleneck is an alternative to the conventional cross-entropy loss and backpropagation that has a number of distinct advantages. It mitigates exploding and vanishing gradients, resulting in the ability to learn very deep networks without skip connections. There is no requirement for symmetric feedback or update locking. We find that the HSIC bottleneck provides performance on MNIST/FashionMNIST/CIFAR10 classification comparable to backpropagation with a cross-entropy target, even when the system is not encouraged to make the output resemble the classification labels. Appending a single layer trained with SGD (without backpropagation) to reformat the information further improves performance.

==> source/sec_NOTES.tex <==
\section*{NOTES/discussion}

%----------------------------------------------------------------

\subsection{Next}

\begin{itemize}
    \item hsic autoencoder.  From Kurt's mail 26nov: "this is the new thought to extend the work we've done into unsupervised learning, and practically the AE or VAE can be directly to test. but today's meeting bastiaan mentioned a big thing about the objective: \\

HSIC-Bottleneck(X, Y, Z) = nHSIC(X,Z) - c * nHSIC(Y,Z)\\
in an unsupervised sense, there's no Y, so then\\
HSIC-Bottleneck(X, Z) = nHSIC(X,Z) - c * nHSIC(X,Z)\\
which makes no sense to apply on the work

my quick thought is by splitting the hsic-bottleneck objective to encoder and decoder respectively:

HSIC-Bottleneck(X, Z) = nHSIC(X, Z)     \# for all Z in encoder as usual\\
$HSIC-Bottleneck(X, Z) = - c * nHSIC(X, Z')$      \# for all Z in decoder but produced from Z\_latent+prior \\

where Z' ~ decoder(Z\_latent + N(0, I)) by introducing some prior or add more information

Bastiaan: Yes, adding noise in the latent layer would be interesting. Some issues:\\
Without constraining the variance or something else the signal Z would blow up so that the noise becomes negligible. So an additional term is needed.\\
Except for the previous issue, it would seem the objective nHSIC(X, Z’) is sufficient. That is, the encoder term is not really needed for the objective, the noise does that job.You would still want to optimise the encoder without backpropagation, but minimizing HSIC(X,Z) is not optimal.

    \item bio-plausible train and then add layer, train. Nothing is lost this way, and training might actually be faster
    \item David's idea, maximize hsic to the next layer.  hmm, now I don't understand
\end{itemize}

\subsection*{Addressed comments:}

 BK: not sure I know what category accuracy is. I would say we are not worried about space at this time.  JP: think this was addressed, I don't see "category accuracy" any more (in first paragraph of section 3)

BK: (re biological plausability, former first paragraph of related work) "I think this paragraph is far too prominent. It can only be this prominent if we then later present our method as a solution to this problem. (Also, Hinton does not think this is a problem.) So we need a more general motivation: what is bad about backpropagation in general (complex, needs lots of data)."\\
\JP{reordering so that this is the 3rd paragraph}
    
BK: "That is a good point that is not exploited: with the information bottleneck we can prevent overfitting which conventional dNN cannot."\\
There is now a sentence in the introduction that mentions this, contributions section:
\JP{"Because the network training is explicitly based on an IB principle, it addresses overfitting by design."}

BK: "a sentence about performance of such (random weights) systems"
\JP{added}

%----------------------------------------------------------------
\subsection*{TODO}
\begin{itemize}

\item check on AAAI sections usage

\item look at NTK - is there a relation?

\item for arxiv:  In setion 3.2 Unformated training:  "This is done by setting the dimensionality fo the last layer $Z_L$ to match the number of classes".  a) $Z_L$ not bold is not defined,
b) bold $\ZZ_L$ is defined, but includes the minibatch size, so would be wrong here.  

\item intro, add sentence emphasizing that the comparisons are fair/identical architectures even if the results are not SoTA

\item make sure we say: IB doesn't have overfitting,
though you need to pick the right lambda

\item results did not make use of extensive hyperparameter search

\item cite these: Kohan error forward propagation, decoupled greedy learning, 
difference target propagation, kernel target alignment
whittington Theories of Error Back-Propagation in the brain,
kolchinsky CaveatsForInformationBottleneckInDeterministicScenarios, 
wu Learnability,

\item fano

\item this text (section HSIC-bottleneck below eq7) is slightly redundant, stated earlier
"The formulation(6),(7)suggests that the optimalhidden representationZifinds a balance between in-dependence from unnecessary details of the input anddependence with the output. Ideally, the informationneeded to predict the label is retained when(6)con-verges, while unnecessary information that would permitoverfitting is removed"

Also this sentence at the beginning of the Format Training results,
"An interesting question regarding deep neural networksis how effectively these stacked layers learn the informa-tion from the input and the label. "

\item frenkel learning without feedback: direct random target projection:
``Direct feedback alignment (DFA) [14] builds on these results and directly propagates the error between the network predictions and the targets to each hidden layer through fixed random connectivity matrices.
...while using the output error as a global modulator and keeping weight information local. Therefore, DFA bears important structural similarity with learning rules that are believed to take place in the brain, known as three-factor synaptic plasticity rules [17], which rely on local pre-synaptic and post-synaptic spike-based activity together with a global modulator.''

(why) cite The Description Length of Deep Learning Models

tschannen: "For example, MI is notoriously hard to estimate, and using it as an objective for representation learning may lead to highly entangled representations due to its invariance under arbitrary invertible transformations. Nevertheless, these methods have been repeatedly shown to excel in practice. In this paper we argue, and provide empirical evidence, that the success of these methods might be only loosely attributed to the properties of MI, and that they strongly depend on the inductive bias in both the choice of feature extractor architectures and the parametrization of the employed MI estimators."


\item use "backward-locking" term, add to abstract+conclusion

\item cite description length of deep learning models r.e. info theory has been applied to DNN

\item pull bio-plausibility from this paper, which is similar in terms of gross information flow:  
frenkel Learning Without Feedback Direct Random Target Projection As A Feedback alignment Algorithm With Layer wise Feedforward Training

\item more clearly say that this is not the only non-backprop method, include methods motioned in https://www.analyticsindiamag.com/lets-not-stop-at-back-prop-check-out-5-alternatives-to-this-popular-deep-learning-technique/

\item more clearly say comparing against vanilla dense (not conv) baseline, no data augmentation

\item this statement from the introduction: 
a) it sounds contrary to the IB principle,
b) because IB training is used (in particular, independence
with the input is maximized), I am not sure we can really say that more relevant information is retained? 
\emph{Interestingly, the layer dimensionality is highly correlated with the amount of relevant information retained by the network. In Section \ref{s:proposed}, we show that higher dimensionality of the network leads to higher accuracy in the post-training.}
JPmargin: this seems a bit contrary to IB BKmargin:I agree, probably better to not put this here, it is a detail.


\item the Direct Feedback Alignment paper is a precedent for feeding global error directly back to individual layers.
(c.f. whittington Theories of Error Back-Propagation in the brain)

\item change pre-training to hsic-training
\item citations about no parallel weight updates across layers:
"Moreover, back-propagation does not apply directly to non-differentiable nonlinearities and does not allow parallel weight updates across the layers (Le et al., 2011; Carreira-Perpiñán \& Wang, 2014; Taylor et al., 2016).

Also, besides its computational issues, backprop is often criticized from a neuroscience perspective as a biologically implausible learning mechanism (Lee et al., 2015; Bartunov et al., 2018; Krotov \& Hopfield, 2019; Sacramento et al., 2018; Guerguiev et al., 2017), due to multiple factors includ-ing the need for "a distinct form of information propagation (error feedback) that does not influence neural activity, and hence does not conform to known biological feedback mech-anisms underlying neural communication" (Bartunov et al., 2018)1.

\item cite Lilicrap 2016 nature paper rather than 2014 version
%\item is it anonymous review?  remove our names
\item Figure with 1 neuron bottleneck -
argue that SGD training has a hard time pushing to the "shoulders" of the sigmoid due to vanishing gradient 
\KM{Put in \\ref{img:vizc}}

// done:   mention in intro and/or conclusion: can help with vanishing gradient

\item precedents for using simple datasets:
Probabilistic Deep Learning using Random Sum-Product Networks,
kingma ICA/VAE paper.
gradient target prop paper also shows 40\% on cifar.
gradient target prop: ``While the performance on CIFAR-10 is low, this issue is related to the neural network architecture (the ones trained here are feed-forward) rather than the technique itself, since backpropagation
also leads to the same order of performance.'''

\item term ``format training'' - a generalized rotation to extract target info. add to introduction
  
\end{itemize}

%----------------------------------------------------------------
\subsection*{Possible explanation of the one-hot behavior}

Bastiaan: I understand the reasoning except for the “longer” part. I would think what you want is the matrices $K_Z$ and $K_Y$ to be the same except for a gain, which you want to maximise. So-far so good, ignoring the gain that explains what we get, but we don’t know the natural normalization of the matrices (I don’t, I should say); what happens to the gain when you rotate $K_Z$ so it becomes like $K_Y$. That part I am still confused about.

The entries in each matrix are between 0 and 1 before mean subtraction because they are all $exp(-||x-y||^2)$. (This not considering the normalized form, have not thought about that). The kernel matrix for Y is constant, and its elements are also one of two values - should be 1 on the diagonal, and some small value off-diagonal, before mean subtraction.After mean subtraction all the off diagonal (the majority of each matrix) will be small and negative.The 1 because exp(0)=1.  The small negative is because for distance between any other pair of points is some constant value because the points have one-hot coordinates...so that distance is always sqrt(2) I think,  e..g    x=(0,0,1,0),  y = (1,0,0,0),  distance = sqrt(1+0+0+1) = sqrt(2).  The Y vector in the dot product will besomething like (0.1, 0.1,   1,   0.1, 0.1) where 1 is the value on the diagonal and 0.1 ~= exp(-2).
The Z vector is the non-constant one.  The best it can do to match the Y vector is to also make its values be one-hot.  
(Hmm, maybe the argument can be said more simply.  For one thing, maybe the reference to bachnorm is not even needed, because the exp constrains things!)

The one-hot behavior shown in \Fig~\ref{img:presolveonehot} is unexpected, but might be explained by the following argument. 
The inner products \eqref{eq:hsicdotprod} are maximized by aligning the direction of the vector $k_{\ZZ_L}$ formed from $\ZZ_L$ to the constant vector formed from the labels $\YY$, and by increasing its length (equivalently, increasing the magnitude along each dimension).
Recalling that the mean is subtracted, increasing the magnitude can be split into positive and negative cases. Positive elements are increased when the corresponding pair of points is pushed closer together, reaching the maximum value $k(\xx,\xx)=1$ that occurs when the arguments of the kernel are identical.
The negative values are reduced by pushing points further apart.
Under a constraint on the norm the points (such as is approximately provided by batchnorm), the
distance 
\[
   \| \zz_j - \zz_k \|^2 = \text{constant} - 2 \zz_j^T \zz_k
\]
is maximized if the vectors to the points are orthogonal.
Since coordinates lie in the positive hyperquadrant due to the ReLU, this occurs when the points lie along coordinate axes, i.e. have one-hot coefficients. Recall further that the labels $\YY_i$ are constant and one-hot, so all the off-diagonal element so of the kernel matrix will be negative. In summary, when arbitary growth of the vector $k_{\ZZ_L}$ is inhibited (e.g.~due to batchnorm),
maximizing the HSIC($\ZZ,\YY$) encourages all the off-diagonal $k_{\zz_{i,j}}, i \ne j$ elements of the first vector in  \eqref{eq:hsicdotprod} to be orthogonal, resulting in one-hot behavior.

%\textbf{TO THINK: but the batchsize is usually larger than the dimension (e.g. 10). Does the argument still work?}

\subsection*{One-hot argument - OLDER, check and delete}

The one-hot behavior is unexpected, but might be explained by the following argument. 
The inner products \eqref{eq:hsicdotprod} are maximized by aligning the vector $k_{\ZZ_L}$ formed from $\ZZ_L$ to that fromed from the labels $\YY$, and by increasing its length (equivalently, increasing the magnitude along each dimension). In the positive direction, elements attain a maximum value when the arguments of the kernel $k(\uu,\vv$) are identical.
In the negative direction (recalling that the mean is subtracted), a kernel evaluation takes on smaller values when the distance between the points is larger.
Under a constraint on the length (such as is approximately provided by batchnorm), the summed pairwise distances
\[
   \sum_{j,k} \| \pp_j - \pp_k \|^2 = \text{constant} - 2 \pp_j^T \pp_k
\]
are maximized if the vectors to the points are mutually orthogonal.
Under the constraint that all coordinates lie in the positive hyperquadrant due to the ReLU, this occurs when the points like along coordinate axes, i.e. have one-hot coefficients.

\textbf{TO THINK: but the batchsize is usually larger than the dimension (e.g. 10). Does the argument still work?}

%----------------------------------------------------------------
\subsection*{Pre/post training terms}

\JP{Thinking about what would work in a sentence like this:
 ''This suggests that pre-training to convergence provides better post-training performance.''
\begin{itemize}
\item dependence-trained
\item information-based pre-training (IBP training... gradient descent training.
\item  HSIC pre-training .... gradient descent training 
\item gradient-free pre-training ...   gradient descent training 
\item gradient-free pre-training ...   online training 
\end{itemize}
}
 
 %----------------------------------------------------------------
 \subsection*{Should the HSIC(input,hidden) go up at the beginning of training, or down?}
 
 Possible reasons for it to go up:  
 a) The sigma is ignoring some information, and the network learns to get around this
 
 b) the bias is pushing some information onto the flat area of the ReLU, 
 resulting in loss of information.
 
 \subsection*{unused text}
 \JP{An important question, and topic for future work, is validating these results on more complicated datasets. We did not attempt this because our existing code is written for vanilla feedforward nets and would require modification to handle Resnets and other state-of-the-art architectures. 
TODO We did try it on CIFAR-10. On this problem the vanilla feedforward network has an accuracy of only 40\%, while HSIC pretraining provides a competitive result of XX\%. TODO DETAILS  Nevertheless, more experimentation is needed to validate the generality of the ideas explored in this paper.}
\KM{In section \\ref{ss:resnet} I have tested our approach on Conv-based architecture and ResNet as well. MNIST, Fashion MNIST, CIFAR10 are tested.}


%----------------------------------------------------------------
\subsection*{clarifying backprop}

Consider this picture for notation:  

\includegraphics[width=0.4\textwidth]{img/notes/backprop_discussion}

x = input, y=label,  $\hat{y}$ = network output,  
z=hidden activation being optimized currently (one term in the summation),
V,W = weight matrices,
a,b = other hidden activations.

The gradient of hsic(z,y) with respect to the network weights involves both W and V.   The gradient with respect to W treats V as a constant, no problem there.
However the full gradient of hsic(z,y) with respect to the network weights also involves the gradient with respect to V.

Computing the gradient with respect to V is like  
\[
     \frac{d}{dV} = \frac{dh}{dz}  \cdot \frac{dz}{da} \cdot \frac{da}{dV}
\]
and dz/da involves W.   I want to think about this...

I suspect that you are making a simplification that it does not depend on V, and just updating W?  (jp: From email discussion, I think yes this is true, Kurt is just taking the gradient wrt W and ignoring the V gradient)

If yes, that's ok, but it's a "block coordinate descent" approach,
meaning:  the gradient over the whole network simplifies to directions that include V,W, but you are ignoring the V directions,  and then the V directions get updated separately in a different term of the overall summation.

But there's maybe a problem here:  a conventional network objective (cross-entropy) could also be optimized with block coordinate descent (I think), rather than with backprop.   So is it fair to say without backprop when the statement rests on the use of coordinate descent?  I think maybe it is, but we should think carefully about this.

%\frac{d h}{d \text{(weights)}} = \left( \frac{dh}{dW}, \frac \right)  = \frac{dh}{dz} \frac{dz}{da} \frac{da}{dx} = \frac{dh}{dz} \cdot W \cdot V

\subsection*{Apply to AE}

Kurt: unsupervised learning with our work: say (variational)autoencoder with encoder E(x) and decoder D(z), where x and z are input and latent activation
obviously we'd like E(x) compresses the x, but D(z) retains the information of z. Then the objective becomes,
\[
   \| D(E(x)) - x \| + HSIC-bottleneck(x,z,E,D)
\]
where HSIC term becomes: $nHSIC(x,E(x)) - \beta * nHSIC(z, D(z))$, and also it is independent layer optimization

%----------------------------------------------------------------
\subsection*{Notes on previous methods}

\begin{itemize}
\item alemiMurphy Deep Variational Information Bottleneck. 
Is it only applied as a regularizer?  
See above eq18, seems like it is more like "format" training.
Future work: "putting the VIB objective at multiple or every layer of a network".
\item Kolchinsky\&Wolpert nonlinear information bottleneck - seems very similar to alemi\&Murphy, and closely compares to them. See Amjad\&Geiger section 7 for a discussion.
Seems like it is applying an upper bound to a bottleneck layer, then doing a "format training" to the output. 

\end{itemize}
%----------------------------------------------------------------
\subsection*{Misc comments}

Question: is the resnet experiment the only one that uses a convolutional net?
KM: Yes, before resnet section we're only exercising fully-connected dense network for prove of concept. The resnet section is just merely saying our approach can be applied on the modern architecture, say: resnet and convolution

Note that sigma and lambda are coupled.
Ideally would think of finding the sigma that is tuned to the data, and then search for the right lambda.
However, lambda influences the weights through training, and sigma has to be tuned to the weights, so there is interaction.

quote from Tschannen paper conclusion:
``Given the fundamental issues with the current estimators, one may investigate other notions of divergence between p(x,y) and p(x)p(y)''

\subsection*{training with sigmas}
I had tried few experiments, in general the format-training does not reflect good performance. But it might be due to the parameters, or the sigma initialize values.

==> source/sec_supplement_AAAI.tex <==

\subsection*{Toy \UNFORMATTED\ solve}

\Fig~\ref{img:presolveonehot} shows that \UNFORMATTED\ discriminates class signals with one-hot effect. We did a further experiment based on a simple model sized 784-256-128-64-32-16-8-\textbf{1}  with backpropagation and \UNFORMATTED. As is convention, we appended an output layer $O \in \Reals^{10}$ to the backpropagation model to support the cross-entropy objective. 
This experiment shows how well the \UNFORMATTED\ can separate the signal classes in $\Reals^1$. \KM{Although the results change based on the random seed, we found that \UNFORMATTED\ usually produces better separation than backpropagation (\Fig~\ref{img:needle}).}

%jp: ok, but is this proven? Both \Fig~\ref{img:presolveonehot} and \Fig~\ref{img:needle:b}) gives \POSTTRAINED\ better representations to train with.

%\Fig~\ref{img:needle:b} shows that \UNFORMATTED\ gives clear discriminated classed signals than \Fig~\ref{img:needle:a}, suggesting the clustering effects from \UNFORMATTED\ (both \Fig~\ref{img:presolveonehot} and \Fig~\ref{img:needle:b}) gives \POSTTRAINED\ better representations to train with.

% kma - in supplementary
\begin{figure}[H]
%%\vspace{0.6cm}  % move figure down to match other column
  \centering
  \begin{subfigure}[b]{0.45\linewidth} \label{fig_1}
    \includegraphics[width=\linewidth]{img/fig9a-needle-1d-dist-backprop.pdf}
    \caption{Backpropagation}
    \label{img:needle:a}
  \end{subfigure}
  \hspace{1mm}
  \begin{subfigure}[b]{0.45\linewidth} \label{fig_2}
    \includegraphics[width=\linewidth]{img/fig9b-needle-1d-dist-hsictrain.pdf}
    \caption{\UNFORMATTEDC}
    \label{img:needle:b}
  \end{subfigure}
  \caption{The tanh classed activation in $\Reals^{1}$ distribution of MNIST between backpropagation Fig~\ref{img:needle:a}, and \UNFORMATTED\ Fig~\ref{img:needle:b}. Each curve represents the activation distribution from particular image category. The distribution is generated by Gaussian Kernel Density Estimation (KDE).}
  \label{img:needle}
\end{figure}



\subsection*{Relating HSIC to Entropy}

Although HSIC is a measure of (in)dependence, its exact relation to mutual information has not been established. Mutual information is defined in terms of entropy, and it has been observed that entropy and Fisher information are related as volume and surface area \cite{Cover2006}. 

In this section we outline an informal argument that HSIC is analogously related to diameter, making use of the identity $I(X,X) = H(X)$.  %Since HSIC (the Hilbert-Schmidt Independence Criterion) is analogous to mutual information, can HSIC(X,X) be compared to Shannon entropy?
%Since HSIC involves something like a covariance matrix, \JP{TODO WRONG! it is a cross-covariance, not symmetric} 
The relation of entropy to volume is easily suggested in the case of a multivariate Gaussian RV with covariance matrix $\CC$.  
%First consider the case of the entropy of a multivariate Gaussian RV, 
%which also involves a covariance matrix:
The entropy in this case is $H(X_{\text{gaussian}}) \propto \log \det \CC + \text{constant}$. Here the interpretation as a ``volume'' can be seen through the determinant. For comparison with HSIC (below), note that $\CC$ is symmetric and can be diagonalized with real eigenvalues,
$\det \CC = \det \UU \LLambda \UU^T = \det \LLambda = \prod \lambda_k$.


Turning to HSIC, denoting $\tilde{\KK}_X = \HH \KK_X \HH$ (and similarly for $\YY$, 
the HSIC computation is $\frac{1}{n^2} \tr \tilde{\KK}_X \tilde{\KK}_Y$. 
HSIC(X,X) is thus simply $\frac{1}{n^2} \tr \tilde{\KK}_X^2$, i.e. the squared Frobenious norm of the feature covariance matrix. Now in general $\| \bAA \|_F^2 = \sum \lambda_k^2$ because $\tr \bAA^T \bAA = \tr (\PP \LLambda \PP^{-1})( \PP \LLambda \PP^{-1}) = \tr \PP \LLambda^2 \PP^{-1} = \tr \LLambda^2$, making use of the Jordan normal decomposition
(or eigendecomposition in our case because $\tilde{\KK}_X$ is symmetric). 

In summary, entropy is related to volume, as can be see in the Gaussian case through the presence of the determinant, i.e. the product of the eigenvalues.  HSIC(X,X) is related to the Frobenius norm, which is a \emph{sum} of eigenvalues, i.e.~a ``diameter''.





==> source/sec_supplemental2.tex <==
% \subsection{Sufficient statistics} \label{ss:ssp_ssi}
This section provides all experiments figures mentioned in Section \ref{s:spp}.

\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.3\textwidth} \label{fig_1}
    \includegraphics[width=\textwidth]{img/EPOCH_comparison_acc.pdf}
    \caption{accuracy}
  \end{subfigure}
  \hspace{1mm}
  \begin{subfigure}[b]{0.3\textwidth} \label{fig_2}
    \includegraphics[width=\textwidth]{img/EPOCH_comparison_loss.pdf}
    \caption{loss}
  \end{subfigure}
  %JP:[is the Epoch Index label correct?] \KM:Yes I think so because there's only one training epoch during each experiment. So starting from 0 to epoch 1, but I'm not sure this is the correct way to do.  
  \caption{The performances of post-training with different pre-trained network learned by different epochs. The three experiment are trained with 5, 25, 100 epochs, labeled with ep-005, ep-025, and ep-100. This suggests that \JP{pre-training to convergence provides better post-training performance.}}
  \label{img:ssi}
\end{figure}

% \subsection{The effect of network capacity} \label{ss:ssp_cap}
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{img/FIXHID2_comparison_acc.pdf}
    \caption{Accuracy over training.}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{img/FIXHID2_comparison_sp_acc.pdf}
    \caption{Final accuracy of each task.}
  \end{subfigure}
  \caption{The performance of post-training with the different size of \PRETRAINED\ networks. The experiments labeled with dim-8, dim-16, dim-32, dim-64, and dim-128, is trained with the \PRETRAINED\ network of the dimension of 128 and output dimension of 8, 16, 32, 64, and 128 respectively. This reveals the large capacity network would provide more relevant information to the post-training}
  % jp comment - be careful with this, since the IB principle should be saying that only few dimensions are needed, or limited information somehow.
  \label{img:expcap}
\end{figure}

% \subsection{Multiple HSIC pre-trained networks} \label{ss:ssp_multi}
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{img/COMB_comparison_acc.pdf}
    \caption{accuracy}
    \label{img:expcomb:1}
  \end{subfigure}
  \hspace{1mm}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{img/COMB_comparison_sp_acc.pdf}
    \caption{final accuracy across tasks}
    \label{img:expcomb:2}
  \end{subfigure}
  \caption{The performance of post-training with aggregation pre-trained networks. Each task labeled with sigma-5, sigma-10, sigma-15 is post-trained with the pre-training network of sigma 5, 10, and 15 respectively. The "combine" is using all the former mentioned pre-trained, aggregated with summation to the output layer.}
  \label{img:expcomb}
\end{figure}

% \subsection{Experiments on ResNet} \label{ss:ssp_resnet}
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.32\textwidth} 
    \includegraphics[width=\textwidth]{img/MOREMNIST10_comparison_acc.pdf}
    \caption{MNIST dataset}
    \label{img:expres:1}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth} 
    \includegraphics[width=\textwidth]{img/MOREFMNIST10_comparison_acc.pdf}
    \caption{Fashion MNIST dataset}
    \label{img:expres:2}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth} 
    \includegraphics[width=\textwidth]{img/MORECIFAR10_comparison_acc.pdf}
    \caption{CIFAR10 dataset}
    \label{img:expres:3}
  \end{subfigure}
  \caption{ResNet experiment on several datasets. In this experiment, we evaluate our work and conventional backpropagation on ResNet of 5 residual blocks. Both shows our result (labeled with ResNet-Post) is outperform the standard backpropagation training (labeled with ResNet-Backprop) at a few beginning of batch updates and final first epoch.
  \JP{The CIFAR10 result is well below state-of-the-art performance, because we are not using a convolutional architecture. Nevertheless, HSIC pretraining provides a significant boost in performance.}
  }
  \label{img:expres}
\end{figure}

